Roulette: A Semantic Privacy-Preserving Device-Edge Collaborative Inference Framework for Deep Learning Classification Tasks

Deep learning classifiers are crucial in the age of artificial intelligence. The device-edge-based collaborative inference has been widely adopted as an efficient framework for promoting its applications in IoT and 5G/6G networks. However, it suffers from accuracy degradation under non-i.i.d. data distribution and privacy disclosure. For accuracy degradation, direct use of transfer learning and split learning is high cost and privacy issues remain. For privacy disclosure, cryptography-based approaches lead to a huge overhead. Other lightweight methods assume that the ground truth is non-sensitive and can be exposed. But for many applications, the ground truth is the user's crucial privacy-sensitive information. In this paper, we propose a framework of Roulette, which is a task-oriented semantic privacy-preserving collaborative inference framework for deep learning classifiers. More than input data, we treat the ground truth of the data as private information. We develop a novel paradigm of split learning where the back-end DNN is frozen and the front-end DNN is retrained to be both a feature extractor and an encryptor. Moreover, we provide a differential privacy guarantee and analyze the hardness of ground truth inference attacks. To validate the proposed Roulette, we conduct extensive performance evaluations using realistic datasets, which demonstrate that Roulette can effectively defend against various attacks and meanwhile achieve good model accuracy. In a situation where the non-i.i.d. is very severe, Roulette improves the inference accuracy by 21\% averaged over benchmarks, while making the accuracy of discrimination attacks almost equivalent to random guessing.

==> app.tex <==
\appendices
\section{proof of theorem 4.1}
Before proving Theorem 4.1, we first prove the following two theorems.
\begin{thm}
\label{thm:A.1}
Given a input $x$ and a deterministic function $f$, $\left| f(x) \right|\leq B$, $\forall a \in \mathbb{R}^{+}$, the random mechanism $\hat{f}(x)=f(x)+aLap(2B/\sigma)$ is $(\frac{\sigma}{a})$-differentially private.
\end{thm}
\begin{proof}
For any adjacent inputs $x$ and $x^{\prime}$,
\begin{equation}
    \begin{aligned}
        &\quad \frac{\Pr[(f(x)+aLap(2B/\sigma)=S]}{\Pr[(f_{\theta}(x^{\prime})+aLap(2B/\sigma)=S]}\\
        &=\frac{e^{-\frac{\left| S-f(x)\right|\sigma}{2aB}}}{e^{-\frac{\left| S-f(x^{\prime})\right|\sigma}{2aB}}}\\
        &=e^{\frac{\sigma}{2aB}(\left|S-f(x^{\prime})\right|-\left|S-f(x)\right|)} \\
        &\leq e^{\frac{\sigma}{2aB} \left| f(x)-f(x^{\prime})\right|} \\
        &\leq e^{\frac{\sigma}{2Ba} \cdot 2B} = e^{\frac{\sigma}{a}}.
    \end{aligned}
\end{equation}
Based on the Definition 2.1, the $\hat{f}(x)$ is $(\frac{\sigma}{a})$-differentially privacy.
\end{proof}

\begin{thm}
\label{thm:A.2}
Given a input $x\in\mathbb{R}^{p}$, and an arbitrary nullification matrix $I_p\stackrel{R}\gets\{0,1\}^p$ with nullification rate $\eta$, if $\hat{f}(x)$ is a $\epsilon$-differential private mechanism, then $\hat{f}(x\odot I_p)$ is a $\varepsilon$-differentially privacy mechanism where
\begin{equation}
    \varepsilon=\ln\left[(1-\eta)e^{\epsilon} +\eta \right].
\end{equation}
\end{thm}
\begin{proof}
Assuming there are two adjacent inputs $x_1$ and $x_2$ differing only one element $i$, i.e., $x_1=x_2\cup i$. We denote $x_1^{\prime}=x_1\odot I_p,\ x_2^{\prime}=x_2\odot I_p$. There are two possible cases after the operation, i.e., $i\in x_1^{\prime}$ and $i \not\in x_1^{\prime}$. For the first case, it is oblivious that $x_1\odot I_p=x_2\odot I_p$, because the only different element between $x_1$ and $x_2$ are both multiplied by 0. Hence, we have,
\begin{equation}
    \Pr [\hat{f}(x_1\odot I_p)=S] = \Pr [\hat{f}(x_2\odot I_p)=S].
\end{equation}
For the second case, since $\hat{f}$ is $\epsilon$-differentially private, according to Definition 2.1 we have,
\begin{equation}
    \Pr [\hat{f}(x_1\odot I_p)=S] \leq \Pr e^{\epsilon}[\hat{f}(x_2\odot I_p)=S].
\end{equation}
Further, based on the fact that $\Pr[i\not\in x_1^{\prime}]=\eta$, we have,
\begin{equation}
    \begin{aligned}
        &\quad  \Pr [\hat{f}(x_1\odot I_p)=S]\\
        &=\eta\Pr [\hat{f}(x_1\odot I_p)=S]+(1-\eta)\Pr [\hat{f}(x_1\odot I_p)=S]\\
        &\leq \eta\Pr [\hat{f}(x_1\odot I_p)=S]+(1-\eta)e^{\epsilon}[\hat{f}(x_2\odot I_p)=S]\\
        &=\exp{[\ln{(1-\eta)e^{\epsilon}+\eta}]}\Pr [\hat{f}(x_1\odot I_p)=S].
    \end{aligned}
\end{equation}
Again, based on Definition 2.1, we can conclude that $\hat{f}(x\odot I_p)$ is a $\varepsilon$-differentially privacy mechanism where
\begin{equation}
    \varepsilon=\ln\left[(1-\eta)e^{\epsilon} +\eta \right].
\end{equation}
\end{proof}

Then, we prove Theorem 4.1.
\begin{proof}
First of all, we analyze the output of the local net with the proposed Laplace mechanism but without nullification, i.e.,
\begin{equation}
\label{eq:Aouput}
    \begin{aligned}
        \hat{f}(x_l)&=f_\theta^{(2)}\left(f_\theta^{(1)}(x_l)+Lap\left(B/\epsilon\right)\right)\\
        &=f_\theta^{(2)}\left(x_r+Lap\left(B/\epsilon\right)\right).
    \end{aligned}
\end{equation}
Since, generally, $Lap(B/\epsilon)$ is much smaller than $x_r$, we can approximate (\ref{eq:Aouput}) by applying the first-order Taylor series:
\begin{equation}
\label{eq:AApproOut}
    \begin{aligned}
        &\quad f_\theta^{(2)}\left(x_r+Lap\left(B/\epsilon\right)\right)\\
        &\approx f_\theta^{(2)}(x_r)+(\nabla_{x_r} f_\theta^{(2)})^{\textsf{T}}Lap(B/\epsilon)\\
        &=f_\theta(x_l)+(\nabla_{x_r} f_\theta^{(2)})^{\textsf{T}}Lap(B/\epsilon).
    \end{aligned}
\end{equation}
Base on Theorem \ref{thm:A.1}, we can say (\ref{eq:AApproOut}) is $(\epsilon/\Xi)$-differentially private, and $\Xi=\lVert \nabla_{x_r}f_{\theta_t}^{(2)}\rVert_\infty$. Further, by applying the Theorem $\ref{thm:A.2}$, we have,
\begin{equation}
    \varepsilon=\ln\left[(1-\eta)e^{\epsilon/\Xi} +\eta \right].
\end{equation}
\end{proof}


\section{Proof of theorem 4.2}
We provide a hardness of approximation result for finding the ground truth inference function. In particular, we prove unless \textsf{RP=NP}, there is no polynomial time that the attacker can find an approximately ground truth inference function of a two-layer neural network with ReLU activation function under Definition 4.2. The main body of the proof depends on \cite{MixCon}. Formally, consider the inversion problem
\begin{equation}
    f_\theta(x)=x_r,
\end{equation}
where $x_r\in \mathbb{R}^{o}$ is the received hidden layer representation, and without losing generality, we normalize the input into $x \in [-1,1]^p$. $f_\theta$ is the device's net and we consider a two neural network with ReLU activation function, specifically,
\begin{equation}
    f_\theta(x)=W_2\sigma(W_1x+b),
\end{equation}
where $\sigma(\cdot)$ refers to ReLU function, and $W_1\in \mathbb{R}^{m_1\times p},\ W_2\in \mathbb{R}^{m_1\times o},\ b\in\mathbb{R}^{m_1}$ are linear transformation parameters. If an attacker can approximately recover the input data, then it can launch a successful ground truth inference attack. 

First of all, we state necessary definitions and useful related results.
\begin{defn}
\label{3SAT}
(\textsf{3SAT problem}). Given n variables and m clauses in a conjunctive normal form
CNF formula with the size of each clause at most 3, the goal is to decide whether there exists an
assignment to the n Boolean variables to make the CNF formula be satisfied.
\end{defn}
\begin{defn}
(\textsf{MAX3SAT}). Given n variables and m clauses, a conjunctive normal form CNF
formula with the size of each clause at most 3, the goal is to find an assignment that satisfies the
largest number of clauses.
\end{defn}
We use \textsf{MAXE3SAT(Q)} to denote the restricted special case of \textsf{MAX3SAT} where every variable occurs in at most Q clauses, and then we have,

\begin{thm}
(\cite{PreB1}). Unless \textsf{RP=NP}, there is no polynomial time (7/8 + 5$\sqrt{Q}$)-approximate algorithm for \textsf{MAXE3SAT(Q)} .
\end{thm}

Now, we are ready to formally prove the Theorem 4.2.

\begin{proof}
Given an \textsf{3SAT} instance $\omega$ with $n$ variables and $m$ clause, where each variable appears in at most Q clauses, we construct a two layer neural network $f_\omega$ and output representation $x_r$ satisfy the following:
\begin{itemize}
    \item Completeness. If $\omega$ is specifiable, then there exists $x\in[0,1]^{p}$ such that $f_\omega=x_r$
    \item Soundness. For any $x$ such that $\Vert f_\theta (x)-x_r\Vert_2\leq\frac{1}{60Q}\sqrt{o}$, we can recover an assignment to $\omega$ that satisfies at least $(7/8 + 5\sqrt{Q})m$ clauses
\end{itemize}
We set $p=n,\ m_1=m + 200Q^{2}n$ and $o=m+100Q^2n$. For any $j\in[m]$, we use $\omega_j$ to denote the $j$-th clause and use $f_{1,j}(x)$ to denote the output of the $j$-th neuron in the first layer, i.e., $f_{1,j}(x)=\sigma(W_j^{(1)}x+b_j)$, where $W_j^{(1)}$ is the $j$-th row of $W^{(1)}$. For any $i\in[n]$, we use $X_i$ to denote the $i$-th variable.

We use the input $x \in [−1, 1]^n$ to denote the variable, and the first $m$ neurons in the first layer to denote the $m$ clauses. By taking
\begin{equation}
    W_{j,i}^{(1)}=\left\{
    \begin{aligned}
    &1,    &&X_i\in \omega_j;\\
    &-1,      &&\overline{X_i} \in\omega_j;\\
    &0,       && otherwise,
    \end{aligned}
    \right.
\label{eq:GRR2}
\end{equation}
and $b_j=-2$ for any $i\in[n],\ j\in[m]$, and viewing $x_i=1$ as $X_i$ to be false and $x_i=-1$ as $X_i$ to be true. One can verify that $f_{1,j}(x)=0$ if the clause is satisfied, and $f_{1,j}(x)=1$ if the clause is unsatisfied. We simply copy the value in the second layer $f_j(x)=f_{1,j}(x)$ for $j\in[m]$. For other neurons, we make $100Q^2$ copies for each $|x_i (i \in n)|$ in the output layer. This can be achieved by taking
\begin{equation}
\begin{aligned}
    f_{m+(i−1)·100Q^2+k}(x)=&f_{m+(i−1)·100Q^2+k}(x)\\
    &+f_{1;m+100Q^2n+(i−1)·100Q^2+k}(x),
\end{aligned}
\end{equation}
and set
\begin{equation}
\begin{aligned}
    f_{1,m+(i−1)·100Q^2+k}(x)=\max\{ x_i,0\}\\
    f_{1,m+100Q^2n+(i−1)·100Q^2+k}(x)=\max\{ -x_i,0\}.
\end{aligned}
\end{equation}
For any $i\in[n]$, $k\in[100Q^2]$. Finally, we set the target output as
\begin{equation}
    x_r =  (\underbrace{0,...,0}_m, \underbrace{1,...,1}_{100Q^2n})
\end{equation}
We are left to prove the two claims we made about the neural network $f_\theta$ and the target output
$x_r$. For the first claim, suppose $\omega$ is satisfiable and $X=(X_1,...,X_n)$ is the assignment. Then as argued before, we can simply take $x_i=1$ if $X_i$ is false and $x_i=-1$ is $X_i$ is true. One can check that $f_\theta(x)=x_r$.

For the second claim, suppose we are given $x\in[-1,1]^p$ such that
\begin{equation}
    \Vert f_\theta (x)-x_r\Vert_2\le\frac{1}{60Q}\sqrt{o}.
\end{equation}
We start from the simple case when $x$ is binary, i.e., $x \in \{-1, 1\}^{n}$. Again, by taking $X_i$ to be true if $x_i = −1$ and $X_i$ to be false when $x_i = 0$. One can check that the number of unsatisfied clause is at most
\begin{equation}
\begin{aligned}
    \Vert f_\theta (x)-x_r\Vert_2^2&\le\frac{1}{3600Q^2}o\\
    &=\frac{1}{3600Q^2}(m+100Q^2n)\\
    &\le \frac{1}{12}m+\frac{1}{3600Q^2}m\\
    &\le\frac{1}{8}m-\frac{5}{\sqrt{Q}}m.
\end{aligned}
\end{equation}
The third step follows from $n ≤ 3m$, and the last step follows from $Q ≥ 15000$.

Next, we move to the general case that $x\in[-1,1]^{p}$. We would round $xi$ to −1 or +1 based on
the sign. Define $\overline{x}\in\{-1,1\}^n$ as
\begin{equation}
    \overline{x_i}=\arg \min_{t\in\{-1.1\}}|t-x_i|.
\end{equation}
We prove that $\overline{x}$ induces an assignment that satisfies $\left(\frac{7}{8}+\frac{5}{\sqrt{Q}}\right)m$ clauses. It suffices to prove
\begin{equation}
    \Vert f_\theta (\overline{x} )-x_r\Vert_2^2-\Vert f_\theta (\overline{x} )-x_r\Vert_2^2\le\frac{3}{100}m,
\end{equation}
since this implies the number of unsatisfied clause is bounded by
\begin{equation}
\begin{aligned}
     \Vert f_\theta (\overline{x} )-x_r\Vert_2^2&\leq(\frac{1}{12}m+\frac{1}{36Q^2}m)+\frac{3}{100}m\\
     &\leq \frac{1}{8}m-\frac{5}{\sqrt{Q}}m.
\end{aligned}
\end{equation}
The last step follows from $Q\ge10^7$.
Further, we define $\delta_i:=|\overline{x}-x_i|=1-|x_i|\in[0,1]$ and $T:=m+128Q^2n$. Then we have
\begin{equation}
    \begin{aligned}
        &\quad\Vert f_\theta (\overline{x} )-x_r\Vert_2^2-\Vert f_\theta (\overline{x} )-x_r\Vert_2^2\\
        &=\sum_{j=1}^{T}(f_j(\overline{x}-x_{rj}))-(f_j(x)-x_{rj})^2\\
        &=\sum_{j=1}^{m}(f_j(\overline{x})-x_{rj})^2-(f_j(x)-x_{rj})^2\\
        &\quad+\sum_{j=m+1}^{T}(f_j(x)-x_r)^2-(f_i(x)-x_r)^2\\
        &=\sum_{j=1}^{m}f_j(\overline{x})^2-f_j(x)^2-100Q^2\sum_{i=1}^n\delta^2_i\\
        &\le2\sum_{j=1}^{m}|f_{1,j}(\overline{x})-f_{1,j}(x)|-100Q^2\sum_{i=1}^{n}\delta^2_i\\
        &\le2\sum_{j=1}^{m}\sum_{i\not\in\omega_j}\delta_i-100Q^2\sum_{i=1}^{n}\delta^2_i\\
        &\le\frac{n}{100}\\
        &\le\frac{3m}{100}.
    \end{aligned}
\end{equation}
The third step follow from $x_{rj} = 0$ for $j \in [m]$ and for $j \in \{m + 1,· · · , m + 100Q^2n\}, x_{rj} = 1, \vert f_j(\overline{x}) − x_{rj}\vert_2 = 0$ and$ f_j(x) − x_{rj}\vert_2 = \delta_i $ given $j\in[m + (i − 1) · 100Q^2 + 1, i\cdot100Q^2]$. The fourth step follows from that $f_j(x) = f_{1,j}(x)\in[0,1]$ for $j\in[m]$. The fifth step follows from the 1-Lipschitz continuity of the ReLU. The sixth step follows from each variable appears in at most $Q$ clause. This concludes the second claim.
\end{proof}


